Diverse Shape Completion via Style Modulated Generative Adversarial Networks

Shape completion aims to recover the full 3D geometry of an object from a partial observation. This problem is inherently multi-modal since there can be many ways to plausibly complete the missing regions of a shape. Such diversity would be indicative of the underlying uncertainty of the shape and could be preferable for downstream tasks such as planning. In this paper, we propose a novel conditional generative adversarial network that can produce many diverse plausible completions of a partially observed point cloud. To enable our network to produce multiple completions for the same partial input, we introduce stochasticity into our network via style modulation. By extracting style codes from complete shapes during training, and learning a distribution over them, our style codes can explicitly carry shape category information leading to better completions. We further introduce diversity penalties and discriminators at multiple scales to prevent conditional mode collapse and to train without the need for multiple ground truth completions for each partial input. Evaluations across several synthetic and real datasets demonstrate that our method achieves significant improvements in respecting the partial observations while obtaining greater diversity in completions.

==> Figures/stylemodulator.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}{\linewidth}
\begin{center}
    \includegraphics[width=0.95\linewidth]{Figures/Images/stylemodulator.pdf}
\end{center}
\end{subfigure}

\caption{Overview of the style modulator network.  Here $w$ and $b$ are learned weights and biases of a convolution, $w''$ are the demodulated weights, and $A$ is a learned Affine transformation.}
\label{fig:style-modulator}
\end{figure}

==> Figures/teaser.tex <==
\begin{figure}[h]
\centering

\begin{subfigure}{\linewidth}
\centering
\begin{subfigure}{.17\linewidth}
    \includegraphics[width=\linewidth]{Figures/Images/Teaser/cropped-raw.png}
\end{subfigure}
\begin{subfigure}{.17\linewidth}
    \includegraphics[width=\linewidth]{Figures/Images/Teaser/cropped-fake-z3.png}
\end{subfigure}
\begin{subfigure}{.17\linewidth}
    \includegraphics[width=\linewidth]{Figures/Images/Teaser/cropped-fake-z6.png}
\end{subfigure}
\begin{subfigure}{.17\linewidth}
    \includegraphics[width=\linewidth]{Figures/Images/Teaser/cropped-fake-z8.png}
\end{subfigure}
\begin{subfigure}{.17\linewidth}
    \includegraphics[width=\linewidth]{Figures/Images/Teaser/cropped-fake-z1.png}
\end{subfigure}
\end{subfigure} \\


\caption{Diverse completions of a real scanned chair from ScanNet.} 
\label{fig:teaser}
\end{figure}

==> Tables/ablations_old.tex <==
\begin{table}[!htb]
    \begin{minipage}{.5\linewidth}
      \centering
      \caption{Ablation on generator architecture.}
      \vspace{7pt}
      \label{generator_architecture}
        \begin{tabular}{l c c c}
        \toprule
        Method & MMD $\downarrow$ & TMD $\uparrow$ & UHD $\downarrow$ \\
        \midrule
        SF & 1.45 & 3.21 & 3.37 \\
        PE+SF & 1.56 & 3.74 & 3.83 \\
        PE+SF+PC (Ours) & 1.50 & 4.36 & 3.79 \\
        \bottomrule
        \end{tabular}
    \end{minipage}%
    \begin{minipage}{.5\linewidth}
        \centering
        \caption{Ablation on style code generation.}
        \vspace{7pt}
        \label{style_code_generation}
        \begin{tabular}{l c c c}
        \toprule
        Method & MMD $\downarrow$ & TMD $\uparrow$ & UHD $\downarrow$ \\
        \midrule
        Gaussian Noise & 1.57 & 3.71 & 4.59 \\
        Mapping Network & 1.45 & 4.03 & 3.72 \\
        Style Encoder (Ours) & 1.50 & 4.36 & 3.79 \\
        \bottomrule
        \end{tabular}
    \end{minipage} 
\end{table}

==> Tables/discriminator.tex <==
\begin{table}
\caption{Ablation on discriminator architecture.}
\vspace{7pt}
\label{discriminator}
\footnotesize
\centering
\begin{tabular}{l c c c}
\toprule
Method & MMD $\downarrow$ & TMD $\uparrow$ & UHD $\downarrow$ \\
\midrule
Single-scale & 1.58 & 2.05 & 4.27 \\
Multi-scale (Ours) & 1.50 & 4.36 & 3.79 \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/diversity_ablation.tex <==
\begin{table}
\caption{Ablation on different regularization terms for diversity}
\centering
\begin{tabular}{l c c c}
\toprule
Method & MMD $\downarrow$ & TMD $\uparrow$ & UHD $\downarrow$ \\
\midrule
EMD & 1.82 & 7.14 & 6.16 \\
Feat. Diff. (Ours) & 1.50 & 4.36 & 3.79 \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/generator_ablation.tex <==
\begin{table}
\caption{Ablation on completion network architecture}
\centering
\begin{tabular}{l c c c}
\toprule
Method & MMD $\downarrow$ & TMD $\uparrow$ & UHD $\downarrow$ \\
\midrule
SF & 1.45 & 3.21 & 3.37 \\
SF + PE & 1.56 & 3.74 & 3.83 \\
SF + PE + PCI (Ours) & 1.50 & 4.36 & 3.79 \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/loss_ablation.tex <==
\begin{table*}[!htb]
\caption{Ablation on loss functions.}
\label{loss_ablation}
\footnotesize
\centering
\begin{tabular}{l c c c}
\toprule
 & MMD $\downarrow$ & TMD $\uparrow$ & UHD $\downarrow$ \\
\midrule
w/o $\mathcal{L}_{comp}$ & 1.62 & 4.61 & 4.58 \\
w/o $\mathcal{L}_{part}$ & 1.81 & 5.97 & 13.03 \\
w/o $\mathcal{L}_{div}$ & 1.70 & 0.41 & 3.57 \\
Ours & 1.50 & 4.36 & 3.79 \\
\bottomrule
\end{tabular}
\end{table*}

==> Tables/runtime.tex <==
\begin{table*}[!htb]
\caption{Completion inference speeds on a NVIDIA V100.}
\label{runtime}
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l c c c c}
\toprule
 &  KNN-latent \cite{wu_2020_ECCV}  & cGAN \cite{wu_2020_ECCV} & PVD \cite{Zhou_2021_ICCV} & Ours \\
\midrule
Time (ms) & 4.5 & 5 & 44950 & 85 \\
\bottomrule
\end{tabular}
\end{table*}

==> Tables/style_code_ablation.tex <==
\begin{table}
 \centering
 \caption{Ablation on style code generation.}
 \vspace{7pt}
 \label{style_code_generation}
 \footnotesize
 \begin{tabular}{l c c c}
 \toprule
 Method & MMD $\downarrow$ & TMD $\uparrow$ & UHD $\downarrow$ \\
 \midrule
 Gaussian Noise & 1.57 & 3.71 & 4.59 \\
 Mapping Network & 1.45 & 4.03 & 3.72 \\
 Style Encoder (Ours) & 1.50 & 4.36 & 3.79 \\
 \bottomrule
 \end{tabular}
\end{table}

==> Tables/z_ablation.tex <==
\begin{table*}[!htb]
\caption{Ablation on style code dim.}
\label{style_code_ablation}
\footnotesize
\centering
\begin{tabular}{l c c c}
\toprule
Style Code & MMD $\downarrow$ & TMD $\uparrow$ & UHD $\downarrow$ \\
\midrule
512-dim & 1.51 & 3.41 & 3.98 \\
128-dim & 1.54 & 3.30 & 4.17 \\
32-dim & 1.59 & 3.89 & 4.04 \\
16-dim & 1.55 & 3.96 & 3.97 \\
8-dim & 1.51 & 3.94 & 3.97 \\
4-dim & 1.51 & 4.00 & 3.93 \\
8-dim + noise (Ours) & 1.50 & 4.36 & 3.79 \\
\bottomrule
\end{tabular}
\end{table*}
